Co-Learning Empirical Games and World Models

Game-based decision-making involves reasoning over both world dynamics and strategic interactions among the agents. Typically, empirical models capturing these respective aspects are learned and used separately. We investigate the potential gain from co-learning these elements: a world model for dynamics and an empirical game for strategic interactions. Empirical games drive world models toward a broader consideration of possible game dynamics induced by a diversity of strategy profiles. Conversely, world models guide empirical games to efficiently discover new strategies through planning. We demonstrate these benefits first independently, then in combination as realized by a new algorithm, Dyna-PSRO, that co-learns an empirical game and a world model. When compared to PSRO -- a baseline empirical-game building algorithm, Dyna-PSRO is found to compute lower regret solutions on partially observable general-sum games. In our experiments, Dyna-PSRO also requires substantially fewer experiences than PSRO, a key algorithmic advantage for settings where collecting player-game interaction data is a cost-limiting factor.

==> appendices/symbols.tex <==
Bolt typeface refers to the joint across all players.
Subscript is used to denote a specific player $s_i$, or to denote all but a specific player $s_{-i}$.

\begin{center}
\begin{tabular}{ll}
    $h\in\mathcal{H}$ & World state \\ 
    $t\in\mathcal{T}$ & Time \\
    $o\in\mathcal{O}$ & Observation \\
    $a\in\mathcal{A}$ & Action \\
    $r\in\mathcal{R}$ & Reward \\
    $m^\pi\in\mathcal{M}^\pi$ & Agent's memory (recurrent state) \\
    $s\equiv(m^\pi, o)$ & Information State \\
    $\mathcal{S}\equiv(\mathcal{M}^\pi,\mathcal{O})$ & Information-State Space \\
    $(s^t, a^t, r^{t+1}, s^{t+1})$ & Transition or Experience \\
    $\tau$ & Sequence, or trajectory, of experiences. \\
    $\pi:\mathcal{O}\times\mathcal{M}^\pi\to\Delta(\mathcal{A})$ & Policy \\
    $\Pi$ & Policy Space \\
    $\sigma:\Pi\to\mathbb{R}$ & Strategy \\
    $\Sigma$ & Strategy Space \\
    $p:\mathcal{H}\times\mathbfcal{A}\to\Delta(\mathcal{H})\times\Delta(\mathbfcal{R})$ & Transition dynamics \\
    $U:\bm\Pi\to\mathbb{R}^n$ & Utility function \\ 
    $n$ & Number of players in a game \\
    $\Gamma\gets (\bm\Pi, U, n)$ & Normal-Form Game \\
    $\hat\Gamma\gets (\bm{\hat\Pi}, \hat{U}, n)$ & Empirical Normal-Form Game \\
    $\mathcal{B}$ & Replay Buffer \\
    $m^w\in\mathcal{M}^w$ & World model's memory (recurrent state) \\
    $w:\mathbfcal{O}\times\mathbfcal{A}\times\mathcal{M}^w\to\mathbfcal{O}\times\mathbfcal{R}$ & Agent world model
\end{tabular}
\end{center}

